Building Efficient Deep Neural Networks with Unitary Group Convolutions

We propose unitary group convolutions (UGConvs), a building block for CNNs which compose a group convolution with unitary transforms in feature space to learn a richer set of representations than group convolution alone. UGConvs generalize two disparate ideas in CNN architecture, channel shuffling (i.e. ShuffleNet) and block-circulant networks (i.e. CirCNN), and provide unifying insights that lead to a deeper understanding of each technique. We experimentally demonstrate that dense unitary transforms can outperform channel shuffling in DNN accuracy. On the other hand, different dense transforms exhibit comparable accuracy performance. Based on these observations we propose HadaNet, a UGConv network using Hadamard transforms. HadaNets achieve similar accuracy to circulant networks with lower computation complexity, and better accuracy than ShuffleNets with the same number of parameters and floating-point multiplies.

==> figs/fig-arch2.tex <==
\begin{figure}[t!]
  \hfill
  \begin{minipage}{0.21\textwidth}
    \includegraphics[width=\textwidth]{figs/fig-arch/fig-arch-shufflenet.pdf}
  \end{minipage}
  \hfill
  \begin{minipage}{0.21\textwidth}
    \includegraphics[width=\textwidth]{figs/fig-arch/fig-arch-hadanet.pdf}
  \end{minipage}
  \hfill

  \hfill
  \begin{minipage}{0.21\textwidth}
      \centering
      (a)
  \end{minipage}
  \hfill
  \begin{minipage}{0.21\textwidth}
      \centering
      (b)
  \end{minipage}
  \hfill
  %\hspace{36pt}
  \caption{\BF{CIFAR-10 and ImageNet blocks with UGConvs --} (a) ResNet block from~\cite{he2015resnet}; (b) ShuffleNet block and our proposed HadaNet variant.
  }
  \label{fig:arch}
\end{figure}

==> figs/fig-diag-vs-conv.tex <==
\begin{figure*}[tb]
  \begin{minipage}{0.41\textwidth}
    \includegraphics[width=\textwidth]{figs/fig-diag-conv/fig-circulant2.pdf}
  \end{minipage}
  \hfill
  \begin{minipage}{0.55\textwidth}
    \includegraphics[width=\textwidth]{figs/fig-diag-conv/fig-block-diag-conv2.pdf}
  \end{minipage}

  \begin{minipage}{0.41\textwidth}
      \centering
      (a)
  \end{minipage}
  \hfill
  \begin{minipage}{0.55\textwidth}
      \centering
      (b)
  \end{minipage}
  \vspace{8px}
  
  \begin{minipage}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/fig-diag-conv/fig-group-conv4.pdf}
  \end{minipage}
  \hfill
  \begin{minipage}{0.25\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/fig-diag-conv/fig-block-dft.pdf}
  \end{minipage}
  \hfill
  \begin{minipage}{0.25\textwidth}
  \end{minipage}

  \begin{minipage}{0.55\textwidth}
  \centering
  (c)
  \end{minipage}
  \hfill
  \begin{minipage}{0.35\textwidth}
  \centering
  (d)
  \end{minipage}
  \hfill
  \begin{minipage}{0.5\textwidth}
  \end{minipage}
  
  \caption{\BF{Convolution with a block-circulant weight tensor --} each square represents a feature map or weight filter. (a) conv layer with a block-circulant weight tensor (block size $B=3$); (b) via Equation~\eqref{eqn:circulant}, each circulant sub-tensor decomposes into a diagonal tensor and a pair of DFTs; (c) convolution with the block-diagonal tensor can be reformulated as group convolution with $B=3$ groups; (d) the per-block DFTs can be organized into block-unitary transforms over the feature axis.
  }
  \label{fig:diag-vs-conv}
\end{figure*}

==> tabs/tab-hada-old.tex <==
\begin{table}[tbp]
  \centering
  \caption{\BF{Hadamard vs. Discrete Fourier transforms --} The entries of the DFT matrix are the complex roots of unity. The entries of the Hadamard matrix are $+1$ or $-1$. The last column shows the structure of $\M{P}^*\M{DP}$ where $\M{D}$ is a diagonal matrix and $\M{P}$ is the transform; differences are bolded.
  }
    \begin{tabular}{ccc}
    \toprule
    \textbf{Transform} & \textbf{Matrix} & \textbf{Wt Structure} \\
    \toprule
    DFT & $\begin{bmatrix} 1 & 1 & 1 & 1 \\ 1 & \omega & \omega^2 & \omega^3 \\ 1 & \omega^2 & \omega^4 & \omega^6 \\ 1 & \omega^3 & \omega^6 & \omega^9 \end{bmatrix}$ &  $\begin{bmatrix} a & b & c & d \\ d & a & b & c \\ c & d & a & b \\ b & c & d & a \end{bmatrix}$ \\
    \midrule
    Hadamard & $\begin{bmatrix} 1 & 1 & 1 & 1 \\ 1 & -1 & 1 & -1 \\ 1 & 1 & -1 & -1 \\ 1 & -1 & -1 & 1 \end{bmatrix}$ & $\begin{bmatrix} a & b & c & d \\ \BF{b} & a & \BF{d} & c \\ c & d & a & b \\ \BF{d} & c & \BF{b} & a \end{bmatrix}$ \\
    %\vspace{2pt}
    \bottomrule
    \end{tabular}%
    \label{tab:hadamard}%
\end{table}
